The FAST Galactic Plane Pulsar Snapshot Survey: II. Discovery of 76 Galactic rotating radio transients and their enigma

We are carrying out the GPPS survey by using the FAST, the most sensitive systematic pulsar survey in the Galactic plane. In addition to about 500 pulsars already discovered through normal periodical search, we report here the discovery of 76 new transient radio sources with sporadic strong pulses, detected by using the newly developed module for a sensitive single pulse search. Their small DM values suggest that they all are the Galactic RRATs. More radio pulses have been detected from 26 transient radio sources but no periods can be found due to a limited small number of pulses from all FAST observations. The following-up observations show that 16 transient sources are newly identified as being the prototypes of RRATs with a period already determined from more detected sporadic pulses, 10 sources are extremely nulling pulsars, and 24 sources are weak pulsars with sparse strong pulses. On the other hand, 48 previously known RRATs have been detected by the FAST. Except for 1 RRAT with four pulses detected in a session of five minute observation and 4 RRATs with only one pulse detected in a session, sensitive FAST observations reveal that 43 RRATs are just generally weak pulsars with sporadic strong pulses or simply very nulling pulsars, so that the previously known RRATs always have an extreme emission state together with a normal hardly detectable weak emission state. This is echoed by the two normal pulsars J1938+2213 and J1946+1449 with occasional brightening pulses. Though strong pulses of RRATs are very outstanding in the energy distribution, their polarization angle variations follow the polarization angle curve of the averaged normal pulse profile, suggesting that the predominant sparse pulses of RRATs are emitted in the same region with the same geometry as normal weak pulsars.

==> KnowRRATs/KnowRRATs.tex <==
\clearpage

\section{Known RRATs}

Some RRATs have observed by FAST.
Based on the strong sensitivity of the telescope, we can get more details of RRATs.

RRAT J0302$+$2252 was discovered at 111 MHz by \citet[][name as J0303$+$2248]{Tyul2016ARep}
and the LOFAR Tied-Array All-Sky Survey (LOTAAS)~\citep[][name as J0302$+$22]{Sanidas2019}.
We used the timing results of \citep{Michilli2020MNRAS} in this paper.
The Figure 5 of \citep{Michilli2020MNRAS} shows that the singlepulses behavior of this pulsar at 149~MHz much like a RRAT or nulling pulsar,
but looking at the pulse-stack of this pulsar in Figure~\ref{Pulse-stacks-K-RRAT1}, it just like ordinary pulsar.

J1853$+$0427, J2000$+$2920, J1843$+$0118, J1905$+$0414 : \citet{Patel2018};
J1905$+$0902, J1928$+$1725 : \citet{Cordes2006};
J0627$+$1612, J0628$+$0909, J1854$+$0306, J1919$+$1745, J1945$+$2357 : \citet{Deneva2009};
J1849$+$0105 : http://www.naic.edu/~palfa/newpulsars/


\begin{table*}
\centering
{\small 
\caption{Previously known RRATs observed by FAST (* indicating new parameters obtained in this paper)}
\centering
\setlength{\tabcolsep}{2.0pt}
\footnotesize
\begin{tabular}{crccclccl}
  \hline\noalign{\smallskip}
    Name     &\multicolumn{1}{c}{P0} & DM       & RA(2000)   & Dec(2000) & ObsDate/MJD: BeamName  & T$_{\rm obs}$& $N_{>3\sigma}$/$N_{all}$       & Notes \\
             &\multicolumn{1}{c}{(ms)}&(cm$^{-3}$pc)&(hh:mm:ss)& (dd:mm)   &                        &  (min) &\%&        \\
  \hline
%J0302$+$2252 & 1207.073!&  19.0 & 03:02:32!&$+$22:52!&20210921/59477: J0302+2252-M01P1    & 15 &$-$6.83(3)*& OP            \\
J1853$+$0427 & 1320.595*& 549.3 & 18:53.46*&$+$04:27*&20200605/59004: G37.24+1.53-M01P2   & 5  & 76.07     & = J1853$+$04  \\ 
J1905$+$0902 &  218.253!& 433.4 & 19:05:19!&$+$09:02!&20200418/58956: G42.77+1.10-M14P4   & 5  & 63.03     & OP            \\  % pulsar
J2000$+$2920 & 3073.698*& 132.5 & 20:00:12*&$+$29:20*&20200222/58901: G66.39-0.34-M08P2   & 5  & 97.12     & = J2000$+$29  \\ 
J0627$+$1612 & 2180.016*& 113   & 06:27:13!&$+$16:12!&20200102/58850: G195.98+2.20-M05P3  & 5  & 33.33     & RRAT          \\ 
J1854$+$0306 & 4557.820!& 192.4 & 18:54:03!&$+$03:06!&20200509/58977: G36.07+1.02-M12P1   & 5  & 44.78     & GP            \\  %
J1905$+$0414 &  894.124*& 383   & 19:05:11!&$+$04:14!&20210624/59388: J190511+041400sp-M01& 15 & 38.27     & RRAT          \\  %
J1928$+$1725 &  289.807*& 136   & 19:28:52*&$+$17:25*&20200421/58959: G52.65-0.25-M17P1   & 15 & 19.39     & = J1927$+$1725\\  
J1945$+$2357 &4717.624*&87.5(2)*& 19:45:48*&$+$23:57*&20200220/58899: G60.43-0.51-M16P2   & 5  & 32.81     & = J1946$+$24  \\ 
J0628$+$0909 & 1241.425!&  88.3 & 06:28:36!&$+$09:09!&20210922/59478: J0628+0909-M01P1    & 15 & 43.45     & NP            \\ %
J1843$+$0118 & 1267.056*& 248   & 18:43:27*&$+$01:18*&20201215/59198: G33.23+2.20-M17P2   & 5  & 60.91     & = J1843$+$01  \\
J1849$+$0105 & 1832.183*& 222   & 18:49:51*&$+$01:05*&20200301/58909: G33.82+0.85-M05P1   & 5  & 46.43     & = J1849$+$0112\\
J1919$+$1745 & 2081.343!& 142.3 & 19:19:43!&$+$17:45!&20210709/59404: G51.82+2.20-M10P4   & 5  & 73.83     & NP            \\  %
    \hline \\
    \multicolumn{8}{l}{}
    \end{tabular}
    }
\end{table*}

\begin{table}
    \centering
    {\small 
    \caption{Properties of Integrated polarization profiles for S/N\textgreater3.0 of singlepulses for RRATs that discovered by GPPS.}
    % \label{sptab1}
    \setlength{\tabcolsep}{2.5pt}
    \begin{tabular}{lrrrrr}
    \hline\noalign{\smallskip}
    Name         & RM            & $W_{eq}$  & $L/I$ & $V/I$ &$|V|/I$\\
                 & (rad m$^{-2}$)& (ms)      & (\%)  & (\%)  &(\%)   \\
    \hline
    J1905$+$0902 & 520(3)*       & 5.8       & 20.7  & 1.7   & 2.2   \\
    J1854$+$0306 & $-$54.3(6)*   & 47.0      & 59.3  & -5.9  & 5.8   \\
    J1905$+$0414 & 1090(3)*      & 50.0      & 63.5  & -4.0  & 11.6  \\
    J1928$+$1725 & 215.6(5)*     & 2.1       & 95.9  & -1.8  & 2.4   \\
    J0628$+$0909 & 129.4(3)*     & 9.4       & 31.4  & 15.9  & 16.7  \\
    J1843$+$0118 & 52(5)*        & 37.9      & 44.5  & -8.8  & 9.0   \\
    J1919$+$1745 & 520.5(5)*     & 19.9      & 41.3  & 2.4   & 3.9   \\
    \hline
    \end{tabular}}
\end{table}  



\begin{figure*}
        \centering
        \includegraphics[width=38mm]{KnowRRATs/J0302+2252_20210921_tracking-M01-P1-c1024b1.ar.zap.Fp.debased.pdf}
        \includegraphics[width=38mm]{KnowRRATs/J0627+1612_G195.98+2.20_20200102_snapshot-M05-P3-c2048b1.Fp.debased.pdf}
        \includegraphics[width=38mm]{KnowRRATs/J0628+0909_20210922_tracking-M01_0011_fn.Czap.zap.Fp.debased.pdf}
        \includegraphics[width=38mm]{KnowRRATs/J1839-0141_20191221_tracking-M01-P1-c1024b1.arzFpr.pdf}\\
        \includegraphics[width=38mm]{KnowRRATs/J1843+0118_G33.23+2.20_20201218_snapshot-M17-P2-c2048b1.Fp.debased.pdf}
        \includegraphics[width=38mm]{KnowRRATs/J1846-0257_20191221_tracking-M01-P1-c1024b1.arzFp.pdf}
        \includegraphics[width=38mm]{KnowRRATs/J1849+0105_G33.82+0.85_20200301_snapshot-M05-P1.Fp.debased.pdf}
        \includegraphics[width=38mm]{KnowRRATs/J1853+0427_G37.24+1.53_20200605_snapshot-M01-P2.Fp.debased.pdf}\\
        % \includegraphics[width=38mm]{KnowRRATs/J1854+0306_20191225_tracking-M01-P1-c1024b1.zap.Fp.pdf}
    \caption{
        Pulse-stacks (main panel), S/N for each pulse (right panel) and integrated profiles (bottom) of known RRATs observed by FAST.
    }
    \label{Pulse-stacks-K-RRAT1}
\end{figure*}
\addtocounter{figure}{-1}
\begin{figure*}
        \centering
        \includegraphics[width=38mm]{KnowRRATs/G36.07+1.02_20200509_snapshot-M12-P1.ar.zap.Fp.debased.pdf}
        \includegraphics[width=38mm]{KnowRRATs/J190511+041400sp_20210624_tracking-M01-P1-c2048b1.ar.r.Fp.b2r.pdf}
        \includegraphics[width=38mm]{KnowRRATs/J1905+0902_G42.77+1.10_20200418_snapshot-M14-P4.Fp.debased.pdf}
        \includegraphics[width=38mm]{KnowRRATs/J1909+06_20191221_tracking-M01-P1-c1024b1.arzFp.debased.pdf}\\
        \includegraphics[width=38mm]{KnowRRATs/J1913+1330_20191216_tracking-M01-P1-c1024b1.arz.FpS.debased.pdf}
        \includegraphics[width=38mm]{KnowRRATs/J1919+1745_20210709_snapshot-M10_0073_fn.Czap.Fp.debased.pdf}
        \includegraphics[width=38mm]{KnowRRATs/J192904+173105_20210514_tracking-M04-P1-c2048b1.Fp.debased.pdf}
        \includegraphics[width=38mm]{KnowRRATs/G60.43-0.51_20200220_snapshot-M16-P2-c2048b1.Fp.pdf}\\
    \caption{
        Pulse-stacks (main panel), S/N for each pulse (right panel) and integrated profiles (bottom) of known RRATs observed by FAST -- {\it continued and end}.
    }
    \label{Pulse-stacks-K-RRAT2}
\end{figure*}
\addtocounter{figure}{-1}
\begin{figure*}
        \centering
        \includegraphics[width=38mm]{KnowRRATs/J2000+2920_G66.39-0.34_20200222_snapshot-M08-P2.Fp.debased.pdf}
    \caption{
        Pulse-stacks (main panel), S/N for each pulse (right panel) and integrated profiles (bottom) of known RRATs observed by FAST -- {\it continued and end}.
    }
    \label{Pulse-stacks-K-RRAT3}
\end{figure*}


% polarization
\begin{figure*}
    \centering
        \includegraphics[width=0.5\columnwidth]{KnowRRATs/J0302+2252_20210921_tracking-M01_0011_fn.CT.f8.RM.SF-pol.pdf}
        \includegraphics[width=0.5\columnwidth]{KnowRRATs/J0628+0909_20210922_tracking-M01_0011_fn.CT.pazi.f8.RM.SF-pol.pdf}
        \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1839-0141_tracking_fn.Czap.x.CT.pazi.f8.RM.SF-pol.pdf}
        \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1843+0118_20201218_snapshot-M17_0025_fn.CT.pazi.f4.RM.SF-pol.pdf}\\
        \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1846-0257_tracking_fn.x.f8.CT.pazi.RM.SF-pol.pdf}
        % \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1854+0306_tracking.CT.pazi.b2f8.pazi.RM-pol.pdf}\\
        \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1854+0306_20200509_snapshot-M12_0001_fn.CT.f4.RM.SF-pol.pdf}
        \includegraphics[width=0.5\columnwidth]{KnowRRATs/J190511+041400sp_tracking-M01_0001_fn.Czap.CT.pazi.f4.RM.SF-pol.pdf}
        \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1905+0902_20200418_snapshot-M14_0072_fn.CT.pazi.b2f4.RM.SF-pol.pdf}\\
        \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1909+0641_tracking.CT.pazi.pazi.b2f8.pazi.RM.SF-pol.pdf}
        \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1913+1330_tracking.CT.pazi.f8.RM.SF-pol.pdf}
        \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1919+1745_20210709_snapshot-M10_0073_fn.Czap.zap.CT.pazi.f4.RM.SF-pol.pdf}
        \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1928+1725_20210514_0001_fn-3-10.Czap.x.CT.pazi.f4.RM.SF-pol.pdf}\\
    \caption{
        Polarization profiles for S/N\textgreater3.0 of singlepulses for known RRATs observed by FAST.
    }
\end{figure*}

% \begin{figure*}
%     \centering
%     \includegraphics[width=0.5\columnwidth]{KnowRRATs/J0627+1612_G195.98+2.20_20200102_snapshot-M05-P3-c2048b1.Fp.debasedb4-prof.pdf}
%     \includegraphics[width=0.5\columnwidth]{KnowRRATs/J0628+0909_G202.34-0.68_20191230_snapshot-M12-P2.Fp.debased-prof.pdf}
%     \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1839-0141_20191221_tracking-M01-P1-c1024b1.arzFpr-prof.pdf}
%     \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1843+0118_G33.23+2.20_20201218_snapshot-M17-P2-c2048b1.Fp.debased-prof.pdf}\\
%     \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1846-0257_20191221_tracking-M01-P1-c1024b1.arzFp.debased-prof.pdf}
%     \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1849+0105_G33.82+0.85_20200301_snapshot-M05-P1.Fp.debased-prof.pdf}
%     \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1853+0427_G37.24+1.53_20200605_snapshot-M01-P2.Fp.debased-prof.pdf}
%     \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1854+0306_20191225_tracking-M01-P1-c1024b1.zap.Fp.debased-prof.pdf}\\
%     \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1905+0902_G42.77+1.10_20200418_snapshot-M14-P4.Fp.debased-prof.pdf}
%     \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1909+06_20191221_tracking-M01-P1-c1024b1.arzFp.debased-prof.pdf}
%     \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1913+1330_20191216_tracking-M01-P1-c1024b1.arz4Fp.debased-prof.pdf}
%     \includegraphics[width=0.5\columnwidth]{KnowRRATs/J192904+173105_20210514_tracking-M04-P1-c2048b1.Fp.debased-prof.pdf}\\
%     \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1946+24_G60.43-0.51_20200220_snapshot-M16-P2-c2048b1.Fp-prof.pdf}
%     \includegraphics[width=0.5\columnwidth]{KnowRRATs/J2000+2920_G66.39-0.34_20200222_snapshot-M08-P2.Fp.debased-prof.pdf}\\
%     \caption{
%         Integrated profiles of SNR$>$3.0 (red line) pulses, all integrated pulses (black line), and integrated pulse for SNR$<$3.0 (blue line) of known RRATs,
%         they are normalized by the peak of the SNR$>$3.0 integrated profiles,
%         except for J1928$+$1725 which we used SNR$>$5.0.
%     }
% \end{figure*}



% Energy
% \begin{figure*}
%     \centering
%     \includegraphics[width=0.5\columnwidth]{KnowRRATs/J0302+2252_20210921_tracking-M01-P1-c1024b1.ar.zap.Fp.debased-Energy.txt-onoff-dis.pdf}
%     \includegraphics[width=0.5\columnwidth]{KnowRRATs/J0627+1612_G195.98+2.20_20200102_snapshot-M05-P3-c2048b1.Fp.debasedb4-Energy.txt-onoff-dis.pdf}
%     \includegraphics[width=0.5\columnwidth]{KnowRRATs/J0628+0909_20210922_tracking-M01_0011_fn.Czap.zap.Fp.debased-Energy.txt-onoff-dis.pdf}
%     \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1839-0141_20191221_tracking-M01-P1-c1024b1.arzFpr-Energy.txt-onoff-dis.pdf}\\
%     \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1843+0118_G33.23+2.20_20201218_snapshot-M17-P2-c2048b1.Fp.debased-Energy.txt-onoff-dis.pdf}
%     \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1846-0257_20191221_tracking-M01-P1-c1024b1.arzrb.Fp-Energy.txt-onoff-dis.pdf}
%     \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1849+0105_G33.82+0.85_20200301_snapshot-M05-P1.Fp.debased-Energy.txt-onoff-dis.pdf}
%     \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1853+0427_G37.24+1.53_20200605_snapshot-M01-P2.Fp.debased-Energy.txt-onoff-dis.pdf}\\
%     % \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1854+0306_20191225_tracking-M01-P1-c1024b1.zap.Fp.debased-Energy.txt-onoff-dis.pdf}\\
%     \includegraphics[width=0.5\columnwidth]{KnowRRATs/J190511+041400sp_20210624_tracking-M01-P1-c2048b1.ar.r.Fp.b2r-Energy.txt-onoff-dis.pdf}
%     \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1905+0902_G42.77+1.10_20200418_snapshot-M14-P4.Fp.debased-Energy.txt-onoff-dis.pdf}
%     \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1909+06_20191221_tracking-M01-P1-c1024b1.arzFp.debased-Energy.txt-onoff-dis.pdf}
%     \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1913+1330_20191216_tracking-M01-P1-c1024b1.arz4Fp-Energy.txt-onoff-dis.pdf}\\
%     \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1919+1745_20210709_snapshot-M10_0073_fn.Czap.Fp.debased-Energy.txt-onoff-dis.pdf}
%     \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1928+1725_G52.65-0.25_20200421_snapshot-M17-P1.Fp.debased-Energy.txt-onoff-dis.pdf}
%     \includegraphics[width=0.5\columnwidth]{KnowRRATs/J1946+24_G60.43-0.51_20200220_snapshot-M16-P2-c2048b1.Fp-Energy.txt-onoff-dis.pdf}
%     \includegraphics[width=0.5\columnwidth]{KnowRRATs/J2000+2920_G66.39-0.34_20200222_snapshot-M08-P2.Fp.debased-Energy.txt-onoff-dis.pdf}\\
%     \caption{
%         Normalized histograms of on- (red line) and off-pulse (blue line) energy of known RRATs observed by FAST.
%     }
% \end{figure*}



\clearpage


==> Tex/Energy-GPPS.tex <==
\clearpage
\begin{table}
    {\small 
    \caption{A list of parameters for new radio sources discovered in GPPS by single pulse search technology.}
    \centering
    \setlength{\tabcolsep}{6.5pt}
    \begin{tabular}{lccccc}
    \hline\noalign{\smallskip}
    % Name            & MJD       & \multicolumn{2}{c}{Log-normal}    & \multicolumn{2}{c}{Power-law/Exponential} \\
    Name            & MJD       & \multicolumn{2}{c}{Log-normal}    & \multicolumn{2}{c}{Power-law/Exp} \\
                    &           & $\mu$     & $\sigma$              &   b           &   c                       \\
    \hline
    J1842$+$0114    & 59289     &  1.63     &   0.64                &   1.14        &   1.27                    \\
    J1845$-$0008    & 59390     &  1.08     &   0.61                &   0.90        &   0.92                    \\
    J1851$+$0051    & 59252     &  3.86     &   0.67                &   0.87        &   0.48                    \\
    J1856$+$0029    & 59357     &  7.65     &   0.63                &   0.45        &   0.20                    \\
    J1857$+$0229    & 59161     &  15.35    &   0.70                &   0.74        &   0.12                    \\
    J1858$+$0453    & 59264     &  8.79     &   0.64                &   1.07        &   0.24                    \\
    J1859$+$0251    & 59289     &  6.35     &   0.65                &   1.10        &   0.33                    \\
    J1900$+$0732    & 59390     &  3.62     &   0.75                &   0.97        &   0.52                    \\
    J1903$+$0319    & 59341     &  3.95     &   0.64                &   1.53        &   0.64                    \\
    J1905$+$0156    & 59227     &  3.46     &   0.73                &   0.96        &   0.58                    \\
    J1905$+$0558    & 59391     &  7.51     &   0.68                &   0.48        &   0.19                    \\
    J1905$+$0849    & 59174     &  4.40     &   0.66                &   0.56        &   0.37                    \\
    J1907$+$0555    & 59154     &  8.11     &   0.69                &   0.81        &   0.23                    \\
    J1911$+$1017    & 59176     &  3.77     &   0.68                &   0.71        &   0.43                    \\
    J1916$+$1142b   & 59222     &  7.26     &   0.63                &   0.99        &   0.28                    \\
    J1919$+$1113    & 59227     &  3.36     &   0.64                &   1.08        &   0.61                    \\
    J1921$+$0851    & 59388     &  0.96     &   0.51                &   2.41        &   6.37                    \\
    J1924$+$1446    & 59139     &  9.54     &   0.63                &   0.79        &   0.20                    \\
    J1924$+$2037    & 59173     &  3.92     &   0.63                &   1.13        &   0.56                    \\
    J2030$+$3929    & 59240     &  1.36     &   0.63                &   0.88        &   1.39                    \\
    J2036$+$3506    & 59390     &  2.84     &   0.63                &   0.95        &   0.69                    \\
    \hline
    \end{tabular}
    }
\end{table}

\begin{figure*}
    \centering
        \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J184213+011400sp_20210317_tracking-M01-P1-c2048b1-distribution.pdf}
        \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J184508-000800sp_20210626_tracking-M01-P1-c2048b1.Fp.debased-Energy.txt-Energy-distribution.pdf}
        \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1852+0051_arctracking-M01-P1-c512b1.arzf8Fp.debased-Energy.txt-Energy-distribution.pdf}
        \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1856+0029_20210524_arctracking-M01-P1-c1024b1.Fpr-Energy.txt-Energy-distribution.pdf}\\
        \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1857+0229_20201108_tracking-M01-P1.arzf16Fp.debased-Energy.txt-Energy-distribution.pdf}
        \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1859+0453_tracking-M01-P1-c512b1.arzf8b2Fp.debased-Energy.txt-Energy-distribution.pdf}
        \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1859+0251_tracking-M01-P1-c512b1-Energy-distribution.pdf}
        \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J190015+073203sp_20210626_tracking-M01-P1-c2048b1.ar.zap.Fp.debased.pazi-Energy.txt-Energy-distribution.pdf}\\
        \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1903+0319_20210508_tracking-M01-P1-c1024b1.Fp.debased-Energy.txt-Energy-distribution.pdf}
        \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1905+0156_20210113_tracking-M01-P1-c2048b1.arzf16Fp.debased-Energy.txt-Energy-distribution.pdf}
        \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J190452+060345_20210306_tracking-M03-P1-c2048b1.ar.Fp.debased-Energy.txt-Energy-distribution.pdf}
        \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1905+0849_20201121_tracking-M01-P1.zapFpr.debased-Energy.txt-Energy-distribution.pdf}\\
        \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1907+0555_20201101_tracking-M01-P1.arzFp.debased-Energy.txt-Energy-distribution.pdf}
        \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1911+1017b_20201123_tracking-M01-P1-c2048b1.arzFpb2.debased-Energy.txt-Energy-distribution.pdf}
        \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1917+1142_tracking-M01-P1-c1024b1-J1916+1142b.zapf16Fp.debasedb4-Energy.txt-Energy-distribution.pdf}
        \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J192111+085133sp_20210624_tracking-M01-P1-c2048b1.ar.Fp.debased.pazi-Energy.txt-Energy-distribution.pdf}\\
        \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1924+1446_20201108_arctracking-M01-P1.arzFp.debasedb4-Energy.txt-Energy-distribution.pdf}
        \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1924+2027_20201127_tracking-M17-P1.arzFp.debased-Energy.txt-Energy-distribution.pdf}
        \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J2030+3929_20210126_tracking-M01-P1-c2048b1.arf32b2Fp.debased-Energy.txt-Energy-distribution.pdf}
        \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J203611+350615sp_20210626_tracking-M01-P1-c2048b1.ar.zap.Fpb2.debased.pazi-Energy.txt-Energy-distribution.pdf}\\
    \caption{
        Normalized energy distributions with log-normal (red line) and Pow-law/Exponential (blue line) fitting of some new single pulse sources discovered by GPPS.
    }
\end{figure*}


\begin{figure*}
    \centering
    \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J184213+011400sp_20210317_tracking-M01-P1-c2048b1.arz.zap.Fp.debased-Energy.txt-onoff-dis.pdf}
    % \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1845-0007_G32.01+1.27_20200422_snapshot-M19-P2.zapf32Fp.debased-Energy.txt-onoff-dis.pdf}
    \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J184508-000800sp_20210626_tracking-M01-P1-c2048b1.Fp.debased-Energy.txt-onoff-dis.pdf}
    \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1852+0051_arctracking-M01-P1-c512b1.arzf8Fp.debased-Energy.txt-onoff-dis.pdf}
    \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1856+0029_20210524_arctracking-M01-P1-c1024b1.Fpr-Energy.txt-onoff-dis.pdf}\\
    \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1857+0229_20201108_tracking-M01-P1.arzf16Fp.debased-Energy.txt-onoff-dis.pdf}
    \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1859+0453_tracking-M01-P1-c512b1.arzf8b2Fp.debased-Energy.txt-onoff-dis.pdf}
    \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1900+0252_tracking-M01-P1-c512b1.arz.zapzFp.debased-Energy.txt-onoff-dis.pdf}
    \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J190015+073203sp_20210626_tracking-M01-P1-c2048b1.ar.zap.Fp.debased.pazi-Energy.txt-onoff-dis.pdf}\\
    \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1903+0319_20210508_tracking-M01-P1-c1024b1.Fp.debased-Energy.txt-onoff-dis.pdf}
    \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J190455+062136sp_20210318_tracking-M01-P1-c2048b1.zapFp.debasedb2-Energy.txt-onoff-dis.pdf}
    \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1905+0156_20210113_tracking-M01-P1-c2048b1.arzf16Fp.debased-Energy.txt-onoff-dis.pdf}
    \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J190452+060345_20210306_tracking-M03-P1-c2048b1.ar.Fp.debased-Energy.txt-onoff-dis.pdf}\\
    \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1905+0849_20201121_tracking-M01-P1.zapFpr.debased-Energy.txt-onoff-dis.pdf}
    \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J190649+033508_20210707_tracking-M01-P1-c2048b1.ar.zap.Fp.debased-Energy.txt-onoff-dis.pdf}
    \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1907+0555_20201101_tracking-M01-P1.arzFp.debased-Energy.txt-onoff-dis.pdf}
    \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1911+1017b_20201123_tracking-M01-P1-c2048b1.arzFpb2.debasedb2-Energy.txt-onoff-dis.pdf}\\
    \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1912+1000_20210113_tracking-M01-P1-c2048b1.arzf32Fp.debasedb2-Energy.txt-onoff-dis.pdf}
    \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1917+1142_tracking-M01-P1-c1024b1-J1916+1142b.zapf16Fp.debasedb4-Energy.txt-onoff-dis.pdf}
    \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1917+0834_20210113_tracking-M01-P1-c2048b1.arzf16Fp.debased-Energy.txt-onoff-dis.pdf}
    \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1919+1113_20210113_tracking-M01-P1-c2048b1.arzFp.debasedb2-Energy.txt-onoff-dis.pdf}\\
    \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J192111+085133sp_20210624_tracking-M01-P1-c2048b1.ar.Fp.debased.pazi-Energy.txt-onoff-dis.pdf}
    \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1924+1446_20201108_arctracking-M01-P1.arzFp.debasedb4-Energy.txt-onoff-dis.pdf}
    \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1924+2037_20201120_tracking-M01-P1.arzFp.debased-Energy.txt-onoff-dis.pdf}
    \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1929+1731_20201120_tracking-M01-P1.arzFp.debasedb4-Energy.txt-onoff-dis.pdf}\\
    \caption{
        Normalized histograms of on- (red line) and off-pulse (blue line) energy of the new single pulse sources discovered by GPPS.
    }
\end{figure*}

\addtocounter{table}{-1}

\begin{figure*}
    \centering
    
    \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1940+2203_20210109_tracking-M01-P1-c2048b1.arzFp.debasedb4.debasedr.debased-Energy.txt-onoff-dis.pdf}
    \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J1940+2231_20201123_tracking-M01-P1.arzf16Fp.debasedb2-Energy.txt-onoff-dis.pdf}
    \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J2030+3929_20210126_tracking-M01-P1-c2048b1.arf32b2Fp.debased-Energy.txt-onoff-dis.pdf}
    \includegraphics[width=0.5\columnwidth]{Energy-GPPS/J203611+350615sp_20210626_tracking-M01-P1-c2048b1.ar.zap.Fpb2.debased.pazi-Energy.txt-onoff-dis.pdf}\\
    \caption{
        Normalized histograms of on- (red line) and off-pulse (blue line) energy of the new single pulse sources discovered by GPPS -- {\it continued and end}.
    }
\end{figure*}

==> Tex/fig_Known_Energy.tex <==

\begin{figure*}
    \centering
    \includegraphics[width=0.45\columnwidth]{Energy-Know/J0156+0400_20211210_snapshot-M04-P3-c2048b1.ar.zap.Fp.debased.S-Energy.txt-E-dist.pdf} 
    \includegraphics[width=0.45\columnwidth]{Energy-Know/J0302+2252_20210921_tracking-M01_0011_fn.Czap.SRF-Energy.txt-E-dist.pdf} 
    \includegraphics[width=0.45\columnwidth]{Energy-Know/G193.24+4.24_20190418_snapshot-M06-P3-c2048b1.ar.zap.Fp.b.debased-Energy.txt-E-dist.pdf} %J0630+1933
    \includegraphics[width=0.45\columnwidth]{Energy-Know/J1354+2400_20211209_snapshot-M01-P4-c2048b1.ar.zap.f8.pazi.Fp.debased-Energy.txt-E-dist.pdf}
    \includegraphics[width=0.45\columnwidth]{Energy-Know/J1538+2345_tracking-M01_0011_fn.Czap.SRF-Energy.txt-E-dist.pdf} 
    \includegraphics[width=0.45\columnwidth]{Energy-Know/J1843+0118_G33.23+2.20_20201218_snapshot-M17-P2-c2048b1.Fp.debased-Energy.txt-E-dist.pdf} 
    \includegraphics[width=0.45\columnwidth]{Energy-Know/J1849+0106sp_20211014_swiftcalibration-M01_0012_fn.Czap.SRF-Energy.txt-E-dist.pdf} 
    \includegraphics[width=0.45\columnwidth]{Energy-Know/J1853+0427sp_20211004_tracking-M01_0001_fn.Czap.SRF-Energy.txt-E-dist.pdf} 
    \includegraphics[width=0.45\columnwidth]{Energy-Know/J1856+0912sp_20211009_swiftcalibration-M01_0013_fn.CFp.debased-Energy.txt-E-dist.pdf} 
    \includegraphics[width=0.45\columnwidth]{Energy-Know/J1905+0902_G42.77+1.10_20200418_snapshot-M14-P4.Fp.debased-Energy.txt-E-dist.pdf} 
    \includegraphics[width=0.45\columnwidth]{Energy-Know/J1908+1351sp_swiftcalibration-M01_0013_fn.zap.SRF-Energy.txt-E-dist.pdf} 
    \includegraphics[width=0.45\columnwidth]{Energy-Know/J1909+0641_tracking-M01_0001_fn.Czap.SRF-Energy.txt-E-dist.pdf} 
    \includegraphics[width=0.45\columnwidth]{Energy-Know/J1915+0639sp_20211009_tracking-M01_0001_fn.Czap.SRF-Energy.txt-E-dist.pdf} 
    \includegraphics[width=0.45\columnwidth]{Energy-Know/J1952+3021sp_tracking-M01_0001_fn.Czap.SRF-Energy.txt-E-dist.pdf} 
    \includegraphics[width=0.45\columnwidth]{Energy-Know/J1958+3033sp_20211009_tracking-M01_0001_fn.Czap.SRF-Energy.txt-E-dist.pdf} 
    \includegraphics[width=0.45\columnwidth]{Energy-Know/J2000+2920sp_20211009_tracking-M01_0001_fn.Czap.SRF-Energy.txt-E-dist.pdf}
%    \caption{ Normalized energy distributions for some known RRATs as normal pulsars.
%    }
%    \label{fig:knowEnergy1}
%\end{figure*}
%
%\begin{figure}
%    \centering
    \includegraphics[width=0.45\columnwidth]{Energy-Know/J0103+5354_20210927_snapshotdec-M04_0075_fn.Czap.SRF-Energy.txt-E-dist.pdf} 
    \includegraphics[width=0.45\columnwidth]{Energy-Know/J1839-0141_20211122_tracking-M01-P1-c2048b1.ar.z.sh.Fp.debased-Energy.txt-E-dist.pdf} 
    \includegraphics[width=0.45\columnwidth]{Energy-Know/J192904+173105_20210514_tracking-M04-P1-c2048b1.Fp.debased-Energy.txt-E-dist.pdf} 
%    \caption{ Normalized energy distributions for known RRATs as nulling pulsars.
%    }
%    \label{fig:knowEnergy2}
%\end{figure}
%
%\begin{figure}
%\centering
\includegraphics[width=0.45\columnwidth]{Energy-Know/J0628+0909_20210922_tracking-M01_0011_fn.Czap.R.CFS-Energy.txt-E-dist.pdf} 
\includegraphics[width=0.45\columnwidth]{Energy-Know/J1848+1516_tracking-M01_0001_fn.Czap.SRF.r-Energy.txt-E-dist.pdf} 
\includegraphics[width=0.45\columnwidth]{Energy-Know/J1854+0306_tracking-M01_0011_fn.Czap.SRF-Energy.txt-E-dist.pdf} 
\includegraphics[width=0.45\columnwidth]{Energy-Know/J1913+1330_G47.61+1.19_20201205_snapshot-M16-P2-c512b1.ar.zap.Fp.debased-Energy.txt-E-dist.pdf} 
% \includegraphics[width=0.45\columnwidth]{Energy-Know/J2033+0042_tracking-M01_0001_fn.Czap.SRF-Energy.txt-E-dist.pdf}
\caption{ Normalized energy distributions for known RRATs as generally very weak pulsars with sparse strong pulses.
}
\label{fig:knowEnergy3}
\end{figure*}



==> Tex/fig_Known_SN.tex <==

\begin{figure}
    \centering
    \includegraphics[width=0.45\columnwidth]{SN-Know/J0302+2252_20210921_tracking-M01_0011_fn.Czap.SRF-Energy.txt-SNR-dist.pdf} 
    \includegraphics[width=0.45\columnwidth]{SN-Know/J1849+0106sp_20211014_swiftcalibration-M01_0012_fn.Czap.SRF-Energy.txt-SNR-dist.pdf}
    \includegraphics[width=0.45\columnwidth]{SN-Know/J1853+0427sp_20211004_tracking-M01_0001_fn.Czap.SRF-Energy.txt-SNR-dist.pdf}
    \includegraphics[width=0.45\columnwidth]{SN-Know/J1856+0912sp_20211009_swiftcalibration-M01_0013_fn.Czap.SRF-Energy.txt-SNR-dist.pdf}
    \includegraphics[width=0.45\columnwidth]{SN-Know/J1905+0902_G42.77+1.10_20200418_snapshot-M14-P4.Fp.debased-Energy.txt-SNR-dist.pdf}
    \includegraphics[width=0.45\columnwidth]{SN-Know/J1909+0641_tracking-M01_0001_fn.Czap.SRF-Energy.txt-SNR-dist.pdf}
    \includegraphics[width=0.45\columnwidth]{SN-Know/J1915+0639sp_20211009_tracking-M01_0001_fn.Czap.SRF-Energy.txt-SNR-dist.pdf}
    \includegraphics[width=0.45\columnwidth]{SN-Know/J1952+3021sp_tracking-M01_0001_fn.Czap.SRF-Energy.txt-SNR-dist.pdf}
    \includegraphics[width=0.45\columnwidth]{SN-Know/J1958+3033sp_20211009_tracking-M01_0001_fn.Czap.SRF-Energy.txt-SNR-dist.pdf}
    \caption{S/N distributions for some known RRATs as normal pulsars.
    }
    \label{fig:knowSN1}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=0.45\columnwidth]{SN-Know/J0103+5354_20210927_snapshotdec-M04_0075_fn.Czap.SRF-Energy.txt-SNR-dist.pdf} 
    \includegraphics[width=0.45\columnwidth]{SN-Know/J1839-0141_20211122_tracking-M01-P1-c2048b1.ar.z.sh.Fp.debased-Energy.txt-SNR-dist.pdf}
    \includegraphics[width=0.45\columnwidth]{SN-Know/J192904+173105_20210514_tracking-M04-P1-c2048b1.Fp.debased-Energy.txt-SNR-dist.pdf}
    \caption{S/N distributions for known RRATs as nulling pulsars.
    }
    \label{fig:knowSN2}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=0.45\columnwidth]{SN-Know/J0627+16sp_20211004_tracking-M01-P1-c2048b1.ar.zap.Fp.rb.debased-Energy.txt-SNR-dist.pdf} 
    \includegraphics[width=0.45\columnwidth]{SN-Know/J0628+0909_20210922_tracking-M01_0011_fn.Czap.R.CFS-Energy.txt-SNR-dist.pdf}
    \includegraphics[width=0.45\columnwidth]{SN-Know/J190511+041400sp_20210624_tracking-M01-P1-c2048b1.ar.r.Fp.b2r-Energy.txt-SNR-dist.pdf}
    \caption{S/N distributions for known RRATs as generally very weak pulsars with sparse strong pulses.
    }
    \label{fig:knowSN3}
\end{figure}

